On the impact of dimensionally-consistent and physics-based inner products for POD-Galerkin and least-squares model reduction of compressible flows

Model reduction of the compressible Euler equations based on proper orthogonal decomposition (POD) and Galerkin orthogonality or least-squares residual minimization requires the selection of inner product spaces in which to perform projections and measure norms. The most popular choice is the vector-valued L2({\Omega}) inner product space. This choice, however, yields dimensionally-inconsistent reduced-order model (ROM) formulations which often lack robustness. In this work, we try to address this weakness by studying a set of dimensionally-consistent inner products with application to the compressible Euler equations. First, we demonstrate that non-dimensional inner products have a positive impact on both POD and Galerkin/least-squares ROMs. Second, we further demonstrate that physics-based inner products based on entropy principles result in drastically more accurate and robust ROM formulations than those based on non-dimensional L2({\Omega}) inner products.As test cases, we consider the following well-known problems: the one-dimensional Sod shock tube, the two-dimensional Kelvin-Helmholtz instability and two-dimensional homogeneous isotropic turbulence.

==> hit2d.tex <==

\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/hit2d_projectionErrorRho.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/hit2d_projectionErrorRhoU.pdf}
\end{subfigure}

\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/hit2d_projectionErrorRhoV.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/hit2d_projectionErrorRhoE.pdf}
\end{subfigure}
\caption{Relative projection errors at the final time step for the mass (left), momentum (center), and energy (right) state variables as a function of basis dimension. Results for the dimensional dataset (D1) are shown in boxes, and results for the non-dimensional dataset (D2) in lines.} 
\label{fig:hit2d_pod_fig}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/rhoDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/GalerkinEntropy_K_100_rhoDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/LeastSquaresL2_K_100_rhoDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/LeastSquaresNonDimensionalL2_K_100_rhoDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/ENtropyLeastSquaresEntropy_K_100_rhoDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/ENtropyLeastSquaresNonDimensionalL2_K_100_rhoDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/rhoNonDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/GalerkinEntropy_K_100_rhoNonDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/LeastSquaresL2_K_100_rhoNonDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/LeastSquaresNonDimensionalL2_K_100_rhoNonDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/ENtropyLeastSquaresEntropy_K_100_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/hit2d/ENtropyLeastSquaresNonDimensionalL2_K_100_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\caption{Relative errors for ROMs of the Kelvin Helmholtz problem for the dimensional configuration (a-f) and non-dimensional configuration (g-l). } 
\label{fig:hit2d_rom100_sols}
\end{center}
\end{figure}

% commenting this out because figures are not found

%% \begin{figure}
%% \begin{center}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRho.pdf}
%% \end{subfigure}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoU.pdf}
%% \end{subfigure}

%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoV.pdf}
%% \end{subfigure}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoE.pdf}
%% \end{subfigure}
%% \caption{Relative projection errors at the final time step for the mass (left), momentum (center), and energy (right) state variables as a function of basis dimension. Results for the dimensional dataset (D1) are shown in boxes, and results for the non-dimensional dataset (D2) in lines.}
%% \label{fig:isentropic_vortex_pod_fig}
%% \end{center}
%% \end{figure}


==> isoentropic.tex <==

We first consider model reduction of the isentropic vortex problem, which comprises a vortex propagating uniformly through the spatial domain. The problem is defined on the periodic domain $\physicalDomain \in [-5,5] \times [-5,5]$ and over the time interval required for one full propagation of the vortex $t \in [0,\sqrt{20}/ \| U_{\infty} \|]$. The problem is run at a Mach number of $M_{\infty} = 0.5$ with the initial conditions
$$\rho_0(\x) = \rho_{\infty} f_1^{ \frac{1}{\gamma - 1}}, \; \; u_1(\x) =  u_{\infty} - f_2 x_2, \; \; u_2(\x) =  v_{\infty} + f_2 x_1, \; \; p = p_{\infty} f_1^{ \frac{\gamma}{\gamma - 1}}$$
where $f_2 = \frac{3}{10}\frac{\| U_{\infty} \|}{2 \pi} \exp(\frac{f_0}{2})$,  $f_1 = 1 - \frac{3}{10}^2(\gamma - 1) M_{\infty}^2 \exp(f_0)(8 \pi^2)^{-1}$, $f_0 = 1 - \sqrt{x^2 + y^2}$, and $u_{\infty} = v_{\infty} = \frac{1}{\sqrt{2}} c_{\infty} M_{\infty}.$ We investigate ROMs applied to a dimensional and non-dimensional version of this problem. The dimensional version is obtained by assuming a specific gas constant of $R = 287.05088 \frac{\mathsf{ J}}{\mathsf{kg K}}$, a freestream density of $\rho_{\infty} = 1.225 \frac{\mathsf{kg}}{\mathsf{m^3}}$, and a freestream temperature of $T_{\infty} = 300 \mathsf{K}$. The non-dimensional version is obtained by setting $R=1, \rho_{\infty} = 1$, and $c_{\infty} = 2$. The following table summarizes the relevant parameters which completely define the initial conditions.
\begin{table}[!h]
\begin{center}
\begin{tabular}{ |c|c|c|c| }
\hline
&  $\rho_{\infty}$ & $c_{\infty}$ & $p_{\infty}$ \\ \hline
Non-dimensional & 1 & 2 & 2.857142857142857\\ \hline
Dimensional & 1.225 & 347.2194852370209 & 105491.19956222906\\ \hline
\end{tabular}
\caption{Summary of conditions used for non-dimensional and dimensional isentropic vortex simulations.}
\label{tab:vortexSetup}
\end{center}
\end{table}

The problem is simulated via a discontinuous Galerkin method on an unstructured mesh comprising $2 \times 32^2 =2048$ elements. The solution is represented by tri-Lagrange polynomials of degree $p=2$ on each element, resulting in a scheme with $\nSpace =(p+1)2048 = 6144$ spatial DOFs. The Roe flux is employed at the element interfaces, and the solution is marched in time with a 4th-order Runge--Kutta scheme at a time step size of $\Delta t = 0.1 \frac{10}{32(p+1) c_{\infty}}$, which corresponds to a CFL number of approximately $0.1$. For construction of the POD bases, solutions are saved every $10$th time step, resulting in $\nSnapshots=272$ snapshots.

\subsubsection{POD results}
We first examine the reults of POD performed in the varioua inner products examined in Section~\ref{sec:podInnerProduct}. Figure~\ref{fig:isentropic_vortex_pod_fig} shows the relative errors associated with the various inner products for mass, $x_1$-momentum, and energy. We note that this problem is symmetric, and thus we don't show the $x_2$-momentum. Our numerical results confirm the analysis provided in Section~\ref{sec:podInnerProduct}. The dimensional and non-dimensional $L^2(\Omega)$ inner products result in the same projection errors on each data set up until $K \approx 30$, after which point small discrepancies on the order of $10^{-7}$ can sometimes be observed; we believe this is due to numerical precision. Next, we observe each methodology to result in almost identical results on the dimensional and non-dimensional dataset. A small discrepancy is observed for the $x$-momentum after $K=30$, and we again expect this to be due to numerical precision.

In summary, these results confirm that all three inner products considered in Section~\ref{sec:podInnerProduct} result in bases that provide identical projection errors down to numerical precision, regardless if deployed on a dimensional or non-dimensional dataset.
\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/projectionErrorRho.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/projectionErrorRhoU.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/projectionErrorRhoE.pdf}
\end{subfigure}
\caption{Relative projection errors at the final time step for the mass (left), momentum (center), and energy (right) state variables as a function of basis dimension. Results for the dimensional dataset (D1) are shown in boxes, and results for the non-dimensional dataset (D2) in lines.}
\label{fig:isentropic_vortex_pod_fig}
\end{center}
\end{figure}


\subsubsection{Reduced-order modeling results}
We now consider results of the various ROMs examined in Sections~\ref{sec:galerkin} and~\ref{sec:least_squares} applied to the isentropic vortex problem

\begin{figure}[!t]
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errors_density.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errors_rhou1.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errors_rhoE.pdf}
\end{subfigure}
\caption{Percent change in errors for ROMs applied on the non-dimensional dataset as compared to the dimensional dataset for $K=10$ (left), $K=15$ (center), and $K=20$ (right).}
\label{fig:isentropic_vortex_pod_fig}
\end{center}
\end{figure}


\begin{figure}[!t]
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errorsChange_K10.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errorsChange_K15.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/isentropic_vortex/errorsChange_K20.pdf}
\end{subfigure}
\caption{Percent change in errors for ROMs applied on the non-dimensional dataset as compared to the dimensional dataset for $K=10$ (left), $K=15$ (center), and $K=20$ (right).}
\label{fig:isentropic_vortex_pod_fig}
\end{center}
\end{figure}


==> kh.tex <==
The next example we consider is the Kelvin Helmholtz instability. The problem is governed by the compressible Euler on the periodic domain $\physicalDomain \in [-5,5] \times [-5,5]$ and is run for 2.5 flow through times. The problem is simulated in \href{https://github.com/Pressio/pressio-demoapps}{\textsf{pressio-demoapps}} and is described \href{https://pressio.github.io/pressio-demoapps/euler_2d_kelvin_helmholtz.html}{here}. For spatial discretization we employ a finite volume scheme with Weno5~\ref{} reconstruction on a discrete domain comprising $256$x$256$ uniformly spaced volumes. Time integration is performed with a low-storage RK4 scheme. The initial conditions are:
$$ \left[ \rho, \; u_1, \; u_2, \; p \right] =   \begin{cases} \left[ 2 \rhoInf, \; \frac{1}{2} \uInf, \; 0, \; \frac{7}{2} \pInf  \right] & \x \in \Omega_1 \\ 
\left[ \rhoInf, \; -\frac{1}{2} \uInf, \; 0,\; \frac{7}{2} \pInf \right] & \x \in \Omega_2 \end{cases}$$
where $\Omega_2 =  [-5,5] \times [-2 + \cos( 0.8 \pi x) , 2 + \cos(0.8 \pi x)]$ and $\Omega_1 = \Omega - \Omega_2 $.

We perform two full-order model simulations: a ``non-dimensional" FOM with $\rhoInf = 1, \; \pInf = \frac{1}{\gamma}, \; \uInf = 1$, and a ``dimensional" FOM with $\rhoInf = 1.225,\; \pInf = 101325$ and $\uInf =  \sqrt{ \frac{\gamma \pInf }{\rhoInf} } $. For both cases we run at a CFL of $0.5$ and save snapshots every 5th time step. 

Figure~\ref{fig:kh_pod_fig} presents the projection error as a function of ROM dimension for the various inner products examined in Section~\ref{sec:podInnerProduct}. We observe that $L^2(\Omega)$ inner product results in significantly different bases when applied to the dimensional data vs non-dimensional data. In particular, we observe that the $L^2(\Omega)$ inner product applied to the dimensional dataset results in a bases that has a poor approximation capacity for the density, $x_1$, and $x_2$ momentum fields, but a good approximation capacity for the total energy field. This is an intuitive result as the total energy snapshots are orders of magnitude larger than the density and velocity snapshots and hence dominate the $L^2(\Omega)$ inner product. We next observe that the non-dimensional $L^2_*(\Omega)$ inner product results in bases with equivalent approximation power when applied to the dimensional and non-dimensional data. The same is observed for bases constructed from the entropy inner product. We observe the entropy inner product to result in slightly more accurate bases for the density, $x_1$, and $x_2$ momentum, but a slightly less accurate bases for the total energy. 
\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/kh2d_projectionErrorRho.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/kh2d_projectionErrorRhoU.pdf}
\end{subfigure}

\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/kh2d_projectionErrorRhoV.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/kh2d_projectionErrorRhoE.pdf}
\end{subfigure}
\caption{Relative projection errors at the final time step for the mass (left), momentum (center), and energy (right) state variables as a function of basis dimension. Results for the dimensional dataset (D1) are shown in boxes, and results for the non-dimensional dataset (D2) in lines.} 
\label{fig:kh_pod_fig}
\end{center}
\end{figure}

We next consider the various ROM formulations described above applied to the dimensional and non-dimensional FOMs. Figure~\ref{fig:kh_rom50_errors} depicts the (log of the) relative mean-squared error. We first observe that the Galerkin ROM based on both the dimensional and non-dimensional inner product is unstable. We next observe that the WLS ROMs based on the $L^2(\Omega)$ inner product produces different results for the dimensional and non-dimensional configurations; we observe that the results are significantly worse for the dimensional configuration. This is expected as WLS based on a standard $L^2(\Omega)$ inner product is dimensionally inconsistent. We next observe that the Galerkin ROM based on the entropy inner product, as well as the WLS ROMs based on the $L^2_*(\Omega)$ and entropy inner products produce similar results on both the dimensional and non-dimensional configuration. This is expected, as these ROMs are dimensionally consistent. We observe that the WLS-Entropy ROM with a conserved basis is the most accurate, followed by the WLS-Entropy ROM with an entropy basis, the Galerkin-Entropy ROM, and finally the WLS ROMs with the $L^2_*(\Omega)$ inner product.  

\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errorsDimensional.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errorsNonDimensional.pdf}
\end{subfigure}
\caption{Relative errors for ROMs for the dimensional configuration (left) and non-dimensional configuration (right).} 
\label{fig:kh_rom50_errors}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.7\textwidth}
\includegraphics[trim={0cm 8cm 0 2cm},clip,width=1.0\linewidth]{figures/kelvin_helmholtz/legend.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errors_density.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errors_rhou1.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errors_rhou2.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/errors_rhoE.pdf}
\end{subfigure}
\caption{Convergance of the relative error for various ROMs. Solid lines indicate ROMs applied to the non-dimensional configuration and boxes indicated ROMs applied to the dimensional configuration.} 
\label{fig:kh_convergence}
\end{center}
\end{figure}



We next consider physical space solutions of the various ROMs. Figure~\ref{fig:kh_rom50_sols} presents the density fields predicted by the various ROMs after 2000 time steps for the dimensional configuration (a-f) and non-dimensional configuration (g-l). Note that the Galerkin ROMs based on the $L^2_*(\Omega)$ and $L^2(\Omega)$ inner products are not shown as they went unstable. We observe that the Entropy-based ROMs, which are all dimensionally consistent, provide the best qualitative representation of the flow fields. The WLS ROMs based on the entropy inner products provide the best qualitative representation, followed by the Galerkin-Entropy ROMs. We observe that the WLS ROMs based on the $L^2(\Omega)$ and $L^2_*(\Omega)$ inner products are diffusive and smear the vortex structures occuring in the shear layer. Lastly, we observe that the WLS ROMs based on the standard $L^2(\Omega)$ inner product result in singificantly different solutions for the dimensional and non-dimensional configuration; the solution on the dimensional configuration is particularly poor. This result once again emphasizes the importance of selecting dimensionally consistent inner products. 

\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/rhoDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/GalerkinEntropy_K_25_rhoDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresL2_K_25_rhoDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresNonDimensionalL2_K_25_rhoDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresEntropy_K_25_rhoDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresNonDimensionalL2_K_25_rhoDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/rhoNonDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/GalerkinEntropy_K_25_rhoNonDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresL2_K_25_rhoNonDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresNonDimensionalL2_K_25_rhoNonDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresEntropy_K_25_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresNonDimensionalL2_K_25_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\caption{Relative errors for ROMs of the Kelvin Helmholtz problem for the dimensional configuration (a-f) and non-dimensional configuration (g-l). } 
\label{fig:kh_rom25_sols}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/rhoDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/GalerkinEntropy_K_150_rhoDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresL2_K_150_rhoDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresNonDimensionalL2_K_150_rhoDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresEntropy_K_150_rhoDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresNonDimensionalL2_K_150_rhoDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/rhoNonDimensional.png}
\caption{FOM}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/GalerkinEntropy_K_150_rhoNonDimensional.png}
\caption{Galerkin (Entropy)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresL2_K_150_rhoNonDimensional.png}
\caption{WLS-$L^2(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/LeastSquaresNonDimensionalL2_K_150_rhoNonDimensional.png}
\caption{WLS-$L^2_*(\Omega)$}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresEntropy_K_150_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ entropy basis)}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/ENtropyLeastSquaresNonDimensionalL2_K_150_rhoNonDimensional.png}
\caption{WLS-Entropy (w/ conserved basis)}
\end{subfigure}
\caption{Relative errors for ROMs of the Kelvin Helmholtz problem for the dimensional configuration (a-f) and non-dimensional configuration (g-l). } 
\label{fig:kh_rom150_sols}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/bestRomsDimensional.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.44\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/bestRomsNonDimensional.pdf}
\end{subfigure}
\caption{\% of time a ROM formulation yields a solution with the lowest MSE. Results are compiled over all bases dimensions and state variables.} 
\label{fig:kh_convergence}
\end{center}
\end{figure}

% commenting this out because figures are not found

%% \begin{figure}
%% \begin{center}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRho.pdf}
%% \end{subfigure}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoU.pdf}
%% \end{subfigure}

%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoV.pdf}
%% \end{subfigure}
%% \begin{subfigure}[t]{0.32\textwidth}
%% \includegraphics[clip,width=1.0\linewidth]{figures/kelvin_helmholtz/projectionErrorRhoE.pdf}
%% \end{subfigure}
%% \caption{Relative projection errors at the final time step for the mass (left), momentum (center), and energy (right) state variables as a function of basis dimension. Results for the dimensional dataset (D1) are shown in boxes, and results for the non-dimensional dataset (D2) in lines.}
%% \label{fig:isentropic_vortex_pod_fig}
%% \end{center}
%% \end{figure}


==> kh2.tex <==



==> sod1d.tex <==

In this section, we consider the Sod1D problem. 
This is a typical benchmark problem for compressible Euler ... say more.
The problem is governed by the compressible Euler on the 1D domain 
$\physicalDomain \in [-0.5,0.5]$ and is run for .... 
The problem is simulated using 
\href{https://github.com/Pressio/pressio-demoapps}{\textsf{pressio-demoapps}}, 
see this page: \href{https://pressio.github.io/pressio-demoapps/euler_1d_sod.html}. 
For the spatial discretization we use a finite volume scheme based on Weno5~\ref{} 
reconstruction on a discrete domain comprising $500$ uniformly spaced cells. 
Time integration is performed with a low-storage RK4 scheme. 
The initial conditions are as follows:
% $$ \left[ \rho, \; u_1, \; p \right] =   
% \begin{cases} 
% \left[ \rhoInf, \; 0 \; \pInf \right] & if x < 0 \\ 
% \left[ \rhoInf, \; -\frac{1}{2} \uInf, \; 0,\; \frac{5}{2} \pInf \right] & \x \in \Omega_2 \end{cases}$$
% where $\Omega_2 =  [-5,5] \times [-2 + \cos( 0.8 \pi x) , 2 + \cos(0.8 \pi x)]$ and $\Omega_1 = \Omega - \Omega_2 $.

% We perform two full-order model simulations: a ``non-dimensional" FOM 
% with $\rhoInf = 1, \; \pInf = 1, \; \uInf = \sqrt{\frac{\pInf}{\rhoInf}}$, 
% and a ``dimensional" FOM with $\rhoInf = 1.225,\; \pInf = \frac{5}{2} 101325$ 
% and $\uInf =  \sqrt{ \frac{\pInf }{\rhoInf} } $. 
% In both cases we run at a CFL of $0.25$ and save snapshots every 5th time step. 

\begin{figure}[!t]
\begin{center}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/sod1d/sod1d_projectionErrorRho.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/sod1d/sod1d_projectionErrorRhoU.pdf}
\end{subfigure}
\begin{subfigure}[t]{0.32\textwidth}
\includegraphics[clip,width=1.0\linewidth]{figures/sod1d/sod1d_projectionErrorRhoE.pdf}
\end{subfigure}
\caption{Relative projection errors computed for the 1D Sod problem at the final time step
  for the mass (left), momentum (center), and energy (right) state variables
  as a function of basis dimension. Results for the dimensional dataset (D1)
  are shown in boxes, and results for the non-dimensional dataset (D2) in lines.}
\label{fig:isentropic_vortex_pod_fig}
\end{center}
\end{figure}

